Benchmarking higher-ranking multipoles and polarizability tensors for small molecular systems

Molecular properties govern how molecules interact with one another or external fields. Accurate molecular properties are essential for constructing intermolecular interaction models, and to achieve high accuracy we need to go beyond leading-order (dipolar) terms. This work presents CCSD(T) references for 73 small non-spin-polarized molecules for molecular dipole and quadrupole moments, and dipole-dipole and quadrupole-quadrupole polarizabilities. Using these results, we provide a holistic performance analysis of molecular properties computed with HF, MP2, CCSD, and a wide range of density-functional methods. Additionally, we investigate in detail what levels of basis sets are required to simultaneously describe all properties in the data set. The best-performing density functionals for all four properties are the asymptotically cor- rected hybrid GGAs B97-3-AC, closely followed by PBE0-AC. Surprisingly, modern meta- GGAs and range-separated functionals perform inconsistently, with large errors in the quadrupo- lar properties. These results have direct implications for methods for intermolecular interac- tions, such as symmetry-adapted perturbation theory based on density functional theory, or for the quality of properties and interactions in machine-learning datasets. Finally, for DFT methods, the Jensen aug-pcseg-2 basis set is a computationally efficient alternative to more established basis sets, but for generating correlated references, third-row elements benefit from core polarization, and double augmentation is strictly necessary for quadrupole-quadrupole polarizabilities.

==> utils/packages.tex <==
\RequirePackage{amsmath,euscript,theorem,graphicx,rotating}
\RequirePackage{multicol,multirow}
\RequirePackage{chemformula} % Formula subscripts using \ch{}
\RequirePackage[T1]{fontenc} % Use modern font encodings
%\RequirePackage[latin1]{inputenc}
\RequirePackage[T1]{fontenc}
\RequirePackage{txfonts}
\RequirePackage{url}
\RequirePackage{verbatim}
\RequirePackage[version=4]{mhchem}
\RequirePackage{array}
\RequirePackage{xr} % for eXternal References
\RequirePackage{color}
\RequirePackage{dcolumn}% Align table columns on decimal point
\RequirePackage{bm}% bold math
\RequirePackage{longtable}% To allow splitting tables across multiple pages
\RequirePackage{xspace}% To preserve spaces after macros
\RequirePackage{booktabs}
\RequirePackage{version}
%\excludeversion{omit}
% This is to allow text under images using \stackunder[0pt]{fig}{text}
\RequirePackage{stackengine}
% For additional symbols (inc degree)
\RequirePackage{gensymb}
\bibstyle{achemso}
\RequirePackage[T1]{fontenc}
% \RequirePackage[latin1,utf8]{inputenc} %%% Not necessary with xetex or luatex
% \RequirePackage[ backend=biber,%style=alphabetic,%sorting=ynt
% ]{biblatex}

\RequirePackage[export]{adjustbox}

\RequirePackage{multicol}

\RequirePackage{xr-hyper} % For cross document referencing (recommended by chatgpt). Purpose: getting SI references in main body.
% It is explained here: https://www.overleaf.com/learn/how-to/Cross_referencing_with_the_xr_package_in_Overleaf
% Be cautious with \externaldocument statements: there should be no errors. And you might have to clear cache to get changes.

\RequirePackage{textcomp} % some dependency requires perthousand (but I do not think that's actually used. Importing this pacakges avoids the warning.

\RequirePackage{tabularray}
\RequirePackage{multicol}

==> utils/utils.tex <==
%\RequirePackage{siunitx}
\RequirePackage{amsmath}
\usepackage{siunitx}
\usepackage{xcolor}

\NewDocumentCommand{\com}{m}{\textcolor{gray}{\textit{#1}}}

\NewDocumentCommand{\prc}{m}{\SI{#1}{\%}}


